Sliding down the stairs: how correlated latent variables accelerate learning with neural networks

Neural networks extract features from data using stochastic gradient descent (SGD). In particular, higher-order input cumulants (HOCs) are crucial for their performance. However, extracting information from the $p$th cumulant of $d$-dimensional inputs is computationally hard: the number of samples required to recover a single direction from an order-$p$ tensor (tensor PCA) using online SGD grows as $d^{p-1}$, which is prohibitive for high-dimensional inputs. This result raises the question of how neural networks extract relevant directions from the HOCs of their inputs efficiently. Here, we show that correlations between latent variables along the directions encoded in different input cumulants speed up learning from higher-order correlations. We show this effect analytically by deriving nearly sharp thresholds for the number of samples required by a single neuron to weakly-recover these directions using online SGD from a random start in high dimensions. Our analytical results are confirmed in simulations of two-layer neural networks and unveil a new mechanism for hierarchical learning in neural networks.

==> content/ica.tex <==

\begin{comment}
\subsection{The leading principal and independent components of images are
  correlated}%
\label{sec:pca-vs-ica}

The advantage of the mixed-cumulant model is that the key quantity that controls
the learning speed of the HOCs, the correlation between latent variables
$\rho = \EE \lambda^\mu \nu^\mu$, are easily interpretable and can be measured in real
data.

To estimate $\lambda^\mu$, we simply perform principal component analysis by computing
the leading eigenvector covariance of the inputs. The latent variables $\lambda^\mu$
are then simply given by the projection of each input along that direction. For
even the smallest image data sets like MNIST, computing the leading CP
factor~\cite{kolda2009tensor} of the fourth-order cumulant to obtain the latent
variable $\nu^\mu$ is impossible due to the large number of entries in the
cumulant. While it is possible to estimate the leading CP factors of the
fourth-order \emph{moment} easily, we are not aware of an algorithm that would
estimate the leading CP factor of the \emph{cumulant}. \seb{Check
  again}. Instead, here we resort to an alternative approach where we compute
the first independent component of the images using independent component
analysis~\cite{comon1994independent, bell1995information,
  hyvarinen2000independent}. Most low-dimensional projections~$\lambda$ of
high-dimensional inputs are approximately normally
distributed~\cite{sudakov:1978, diaconis:1984, hall:1993, bobkov:2003,
  meckes:2010aa, reeves:2017c}, so ICA instead looks for linear projections $w$
the inputs that are maximally non-Gaussian by minimising the loss
\begin{equation}
  \label{eq:ica-loss}
 \mathcal L(w) = -{\left[ \EE G(\lambda) - \EE G(\nu) \right]}^2,
\end{equation}
where $G(z)$ is a scalar function of degree at least three, and $\nu$ is a
Gaussian random variable with the same mean and variance as $\lambda$, and the
expectation is computed over a mini-batch of inputs. We implemented a mini-batch
version of the FastICA algorithm of \citet{hyvarinen2000independent} to compute
the leading independent component of the images, using the standard choice
$G(\lambda) = \log \cosh \lambda$.

We show scatter plots of the leading principal and independent components for
three different image data sets in \cref{fig:correlations}. Since the sign of
the leading independent component is undetermined\footnote{Independent component
  analysis assumes a generative model for the inputs as $x = G s$, where $s$ are
  the non-Gaussian ``independent components'' we are seeking, and $G$ is a
  mixing matrix~\cite{hyvarinen2000independent}. Since ICA effectively attempts
  to reconstruct both $G$ and $s$ simultaneously, the sign of the sources is not
  defined.}, we plot the absolute value of the leading independent component
against the leading principal component. We find that \seb{TBD}.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=.33\linewidth]{figs/dummy}%
  \includegraphics[width=.33\linewidth]{figs/dummy}%
  \includegraphics[width=.33\linewidth]{figs/dummy}
  % \captionsetup{format=plain}
  \caption{\label{fig:correlations} \textbf{The leading principal and
      independent component of images are correlated.} We plot the leading
    principal component of different image data sets, computed as the projection
    of the images along the leading eigenvector for the covariance matrix,
    against the leading independent component. The independent component
    $\lambda_{\mathrm{ICA}}$ is obtained by computing the direction
    $w_{\mathrm{ICA}}$ for which the projections
    $\lambda_{\mathrm{ICA}} =  w_{\mathrm{ICA}} \cdot x $ have a
    maxmimally non-Gaussian distribution, as quantified by
    \cref{eq:ica-loss}. Note that inputs are whitened before performing
    independent component analysis, removing any trace of the eigenvectors. We
    computed these independent components using an online version of the FastICA
    algorithm of \citet{hyvarinen2000independent} (see \cref{sec:ica-details}
    for details).}
\end{figure*}
\end{comment}

